Ada-Ranker: A Data Distribution Adaptive Ranking Paradigm for Sequential Recommendation

A large-scale recommender system usually consists of recall and ranking modules. The goal of ranking modules (aka rankers) is to elaborately discriminate users' preference on item candidates proposed by recall modules. With the success of deep learning techniques in various domains, we have witnessed the mainstream rankers evolve from traditional models to deep neural models. However, the way that we design and use rankers remains unchanged: offline training the model, freezing the parameters, and deploying it for online serving. Actually, the candidate items are determined by specific user requests, in which underlying distributions (e.g., the proportion of items for different categories, the proportion of popular or new items) are highly different from one another in a production environment. The classical parameter-frozen inference manner cannot adapt to dynamic serving circumstances, making rankers' performance compromised. In this paper, we propose a new training and inference paradigm, termed as Ada-Ranker, to address the challenges of dynamic online serving. Instead of using parameter-frozen models for universal serving, Ada-Ranker can adaptively modulate parameters of a ranker according to the data distribution of the current group of item candidates. We first extract distribution patterns from the item candidates. Then, we modulate the ranker by the patterns to make the ranker adapt to the current data distribution. Finally, we use the revised ranker to score the candidate list. In this way, we empower the ranker with the capacity of adapting from a global model to a local model which better handles the current task.

==> relatedworks_old.tex <==
relatedworks\section{related works}
%meta learning, model adaption
\subsection{Recommender Systems}
% recall & ranking; shallow to deep because DL good at implicit learning; sequential is a special one; however, no adaption ability;
A web-scale recommender system usually comprises of recall modules and ranking modules to response users' requests in (near) real-time \cite{10.1145/2959100.2959190,ijcai2018-529}. Recall modules propose a small set (such as thousands) of potentially relevant items as candidates with light-weighted models. Ranking modules will score the given item candidates using more advanced models to ensure the final recommendations are accurate. In the past decade, mainstream technologies for rankers have been evolving from shallow models (such as FM~\cite{DBLP:conf/icdm/Rendle10}  and GBDT~\cite{10.1145/2939672.2939785}) to deep learning-based models \cite{10.1145/2959100.2959190,ijcai2018-529,10.1145/2988450.2988454,10.5555/3172077.3172127,10.1145/3219819.3219823} due to the great learning ability of deep neural networks. For example, some work leverages neural networks to learn complex feature interactions~\cite{10.5555/3172077.3172127,10.1145/3219819.3220023,10.1145/3077136.3080777}; DKN incorporates knowledge graph signals into item representation with a knowledge-aware text CNN~\cite{10.1145/3178876.3186175}. 
%\cite{10.1145/3383313.3412236} discusses how to share knowledge effectively across multiple recommendation tasks. 
One important recommendation scenario is the sequential recommendation, where DNNs have been successfully applied, such as GRU4Rec~\cite{DBLP:journals/corr/HidasiKBT15}, NextItNet~\cite{10.1145/3289600.3290975}, and SASRec~\cite{DBLP:conf/icdm/KangM18}. However, all these approaches follow the same traditional train-freeze-test paradigm, where a global optimal model is learned from the training dataset and then freeze the model for testing. The testing environment in recommender systems is highly dynamic with different users' requests, thus, we look for an approach that can perceive the current task's peculiarity and conduct parameter adaptation.

\subsection{Model Adaptation}
Model Adaptation (MA) has recently become a research hotspot in many application fields such as NLP and visual computing. MA aims to maximize the performance on a target task using existing training source data. 
%A source model is usually trained on a large scale dataset and then adapts to specific tasks with few adaptation data. 
Considering that there is a distribution mismatch between training data and testing data, how to leverage the few adaptation data to make the source model generalize to the target task is the key challenge.
Previous works in model adaptation can be roughly divided into two categories.

\textbf{Model Patch.} Finetuning a pre-trained model with target task-specific data is the most common way to transfer knowledge. This work~\cite{DBLP:conf/icml/HoulsbyGJMLGAG19} proposes a parameter-efficient tuning paradigm called \textsl{model patch}, which can adapt a large-scale pre-trained model to a specific downstream task efficiently by finetuning only a small number of new parameters.%, while leaving parameters in the original model unchanged.
PeterRec~\cite{10.1145/3397271.3401156} aims to adapt a user representation model for multiple downstream tasks. It includes a separate grafting neural network (similar to model patch in \cite{DBLP:conf/icml/HoulsbyGJMLGAG19}), which adapts the parameters of convolutional layers in the pre-trained user model to a target task. K-Adapter~\cite{Wang2021KAdapterIK} injects knowledge into large pre-trained models like BERT and RoBERTa with model patch. 

\textbf{Feature Modulation.} 
FiLM~\cite{DBLP:conf/aaai/PerezSVDC18} carries out a feature-wise linear modulation on a neural network's intermediate features conditioned on an arbitrary given input, so that the CNN computation over an image can be influenced by a dynamic condition. TaNP~\cite{10.1145/3442381.3449908} introduces an improved version of FiLM, named Gating-FiLM, to enhance the ability of filtering the information which has the opposite effects during adaptation.  AdaSpeech~\cite{DBLP:conf/iclr/Chen0LLQZL21} adapts few adaptation data to personalized voices, which modulates hidden state vectors in network by categorizing the acoustic conditions in different levels and conditional layer normalization.

\subsection{Multi-task Learning}
Industrial recommender systems usually serve diverse situations. For example, the \textsl{banner} and \textsl{Guess What You Like} channels on Taobao app homepage~\cite{sheng2021model}. To fully learn from the universal data and serve for different situations, a widely adopted method is Multi-task learning (MTL).
MTL optimizes a model by jointly training several related tasks simultaneously. Thanks to the knowledge sharing across related tasks, the model learns a wider perspective for a specific task and can be better generalized. Multi-task learning is typically done with parameter sharing of hidden layers~\cite{DBLP:books/sp/98/Caruana98}. Multi-gate Mixture-of-Experts (MMoE) based models ~\cite{DBLP:conf/kdd/MaZYCHC18,10.1145/3383313.3412236} aim to model task relationships by sharing the expert networks across all tasks, while having a gating network to optimize each task. 
%Note that multi-task learning does not aim to enhance the generalization to a new (unseen) task, MTL contrasts with the domain adaptation problem~\cite{DBLP:journals/ml/Ben-DavidBCKPV10}, where knowledge transfer is a one-way flow, i.e., from the source domain to the target domain. 
Star Topology Adaptive Recommender (STAR)~\cite{sheng2021model} is proposed to train a single model to serve all domains by leveraging data from all domains simultaneously, capturing the characteristics of each domain, and modeling the commonalities between different domains. 
Note that all these MLT methods only work well in the scenario where the tasks/domains are fixed and well-defined, but can hardly generalize to new domains or ad-hoc tasks with dynamic distributions.
